Autoregressive Networks

We propose a first-order autoregressive (i.e. AR(1)) model for dynamic network processes in which edges change over time while nodes remain unchanged. The model depicts the dynamic changes explicitly. It also facilitates simple and efficient statistical inference methods including a permutation test for diagnostic checking for the fitted network models. The proposed model can be applied to the network processes with various underlying structures but with independent edges. As an illustration, an AR(1) stochastic block model has been investigated in depth, which characterizes the latent communities by the transition probabilities over time. This leads to a new and more effective spectral clustering algorithm for identifying the latent communities. We have derived a finite sample condition under which the perfect recovery of the community structure can be achieved by the newly defined spectral clustering algorithm. Furthermore the inference for a change point is incorporated into the AR(1) stochastic block model to cater for possible structure changes. We have derived the explicit error rates for the maximum likelihood estimator of the change-point. Application with three real data sets illustrates both relevance and usefulness of the proposed AR(1) models and the associate inference methods.

==> Autoregressive Networks_updated/QYalias.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%    Resetting of parameters                   %%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
 \renewcommand{\topfraction}{1}
 \renewcommand{\bottomfraction}{1}
 \renewcommand{\textfraction}{0}
 \renewcommand{\floatpagefraction}{0.90}
% \renewcommand{\thefootnote}{\arabic{footnote}}
\renewcommand{\thefootnote}{\fnsymbol{footnote}}
 \@addtoreset{equation}{section}
 \renewcommand{\theequation}{\thesection.\arabic{equation}}
%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%    miscelaneous commands                    %%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \newcommand{\glossaryentry}[2]{\subitem #1 #2}
% \newcommand{\g}[2]{#1\glossary{#1, #2}}
% \renewcommand{\i}[1]{{\em #1 \/} \index{#1} \hspace{-0.05 in}}
% \newcommand{\ii}[1]{{#1} \index{#1} \hspace{-0.05 in}}
% \newcommand{\indexentry}[2]{\item #1 #2}

\newcommand{\HRule}{\rule{\linewidth}{0.3mm}}
\newcommand{\inner}[2]{ \mbox{$ \langle #1, #2 \rangle $} }
\newcommand{\image}[1]{\mbox{Im}(#1)}
\newcommand{\kernel}[1]{\mbox{Ker}(#1)}

\newtheorem{definition}{Definition}[section]
\newtheorem{theorem}{Theorem}
% \newtheorem{theorem}[definition]{Theorem}
\newtheorem{lemma}{Lemma} 
% \newtheorem{lemma}[definition]{Lemma}
%newtheorem{corollary}[definition]{Corollary}
\newtheorem{corollary}{Corollary}
%\newtheorem{proposition}[definition]{Proposition}
\newtheorem{proposition}{Proposition}

% \newtheorem{remarkx}{Remark}[chapter]
% \newenvironment{remark}
% {\begin{remarkx}
% \em}
% {\end{remarkx}}


\renewcommand{\hat}{\widehat}
\def\singlespace{\def\baselinestretch{1}\@normalsize}
\def\endsinglespace{}
\def\endp{{\hfill \vrule width 5pt height 5pt\par}}
\def\wh{\widehat}
\def\wt{\widetilde}
\def\askip{\vspace{0.1in}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  Abbreviations in math mode                   %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\AR}{{\rm AR}}
\newcommand{\MA}{{\rm MA}}
\newcommand{\ARMA}{{\rm ARMA}}
\newcommand{\AAR}{{\rm AAR}}
\newcommand{\ARIMA}{{\rm ARIMA}}
\newcommand{\FAR}{{\rm FAR}}
\newcommand{\ARCH}{{\rm ARCH}}
\newcommand{\GARCH}{{\rm GARCH}}
\newcommand{\Beta}{{\rm Beta}}
\newcommand{\DLS}{{\mbox{\scriptsize DLS}}}
\newcommand{\IRSC}{{\rm IRSC}}
\newcommand{\IID}{{\rm IID}}
\newcommand{\Leb}{{\rm Leb}}
\newcommand{\LK}{{\mbox{\scriptsize LK}}}
\newcommand{\LKopt}{{\mbox{\scriptsize LK, OPT}}}
\newcommand{\LS}{{\mbox{\scriptsize LS}}}
\newcommand{\LSopt}{{\mbox{\scriptsize LS, OPT}}}
\newcommand{\MISE}{{\rm MISE}}
\newcommand{\MSE}{{\rm MSE}}
\newcommand{\STD}{{\rm STD}}
\newcommand{\MSPE}{{\rm MSPE}}
\newcommand{\MAE}{{\rm MAE}}
\newcommand{\MAD}{{\rm MAD}}
\newcommand{\RSS}{{\rm RSS}}
\newcommand{\WN}{{\rm WN}}
\newcommand{\abias}{{\rm AB}}
%\newcommand{\argmin}{{\rm argmin}}
\newcommand{\avar}{{\rm AV}}
\newcommand{\vech}{{\rm vech}}
\newcommand{\bias}{{\rm Bias}}
\newcommand{\cor}{{\rm Corr}}
\newcommand{\cov}{{\rm Cov}}
\newcommand{\diag}{{\rm diag}}
\newcommand{\etal}{\mbox{\sl et al.\;}}
\newcommand{\ie}{\mbox{\sl i.e.\;}}
\newcommand{\eg}{\mbox{\sl e.g.\;}}
\newcommand{\sgn}{{\rm sgn}}
\newcommand{\sopt}{\mbox{{\scriptsize opt}}}
\newcommand{\tr}{{\rm tr}}
\newcommand{\var}{{\rm Var}}
\newcommand{\AIC}{{\rm AIC}}
\newcommand{\BIC}{{\rm BIC}}
\newcommand{\BICP}{{\rm BICP}}
\newcommand{\BICC}{{\rm BICC}}
\def\ga{\gamma}
\def\de{\delta}
\def\om{\omega}
\def\la{\lambda}
\def\vphi{\varphi}
\newcommand{\ve}{{\varepsilon}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  boldface in math model                         %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\bA}{{\mathbf A}}
\newcommand{\bB}{{\mathbf B}}
\newcommand{\bF}{{\mathbf F}}
\newcommand{\bE}{{\mathbf E}}
\newcommand{\bG}{{\mathbf G}}
\newcommand{\bH}{{\mathbf H}}
\newcommand{\bI}{{\mathbf I}}
\newcommand{\bK}{{\mathbf K}}
\newcommand{\bL}{{\mathbf L}}
\newcommand{\bM}{{\mathbf M}}
\newcommand{\bQ}{{\mathbf Q}}
\newcommand{\bP}{{\mathbf P}}
\newcommand{\bR}{{\mathbf R}}
\newcommand{\bS}{{\mathbf S}}
\newcommand{\bU}{{\mathbf U}}
\newcommand{\bV}{{\mathbf V}}
\newcommand{\bW}{{\mathbf W}}
\newcommand{\bX}{{\mathbf X}}
\newcommand{\bY}{{\mathbf Y}}
\newcommand{\bZ}{{\mathbf Z}}
\newcommand{\ba}{{\mathbf a}}
\newcommand{\bb}{{\mathbf b}}
\newcommand{\bd}{{\mathbf d}}
\newcommand{\bc}{{\mathbf c}}
\newcommand{\be}{{\mathbf e}}
\newcommand{\bff}{{\mathbf f}}
\newcommand{\bg}{{\mathbf g}}
\newcommand{\bh}{{\mathbf h}}
\newcommand{\bi}{{\mathbf i}}
\newcommand{\bj}{{\mathbf j}}
\newcommand{\bk}{{\mathbf k}}
\newcommand{\bm}{{\mathbf m}}
\newcommand{\bq}{{\mathbf q}}
\newcommand{\br}{{\mathbf r}}
\newcommand{\bt}{{\mathbf t}}
\newcommand{\bs}{{\mathbf s}}
\newcommand{\bu}{{\mathbf u}}
\newcommand{\bv}{{\mathbf v}}
\newcommand{\bw}{{\mathbf w}}
\newcommand{\bx}{{\mathbf x}}
\newcommand{\by}{{\mathbf y}}
\newcommand{\bz}{{\mathbf z}}
\newcommand{\balpha} {\boldsymbol{\alpha}}
\newcommand{\bbeta}  {\boldsymbol{\beta}}
\newcommand{\bfeta}  {\boldsymbol{\eta}}
\newcommand{\bvarphi}  {\boldsymbol{\varphi}}
\newcommand{\varphiuv}  {\varphi^{(u,v)}}
\newcommand{\bvphi}  {\boldsymbol{\varphi}}
\newcommand{\bBeta}  {\boldsymbol{\Beta}}
\newcommand{\bdelta} {\boldsymbol{\delta}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bepsilon}{\bolsymbol{\varepsilon}}
\newcommand{\bOmega}{\boldsymbol{\Omega}}
\newcommand{\bomega}{\boldsymbol{\omega}}
\newcommand{\bom}{{\boldsymbol{\omega}}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\bDelta}{\boldsymbol{\Delta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\bga}{\boldsymbol{\gamma}}
\newcommand{\bve}{\mbox{\boldmath$\varepsilon$}}
\newcommand{\brho}{\mbox{\boldmath$\rho$}}
\newcommand{\bTheta} {\boldsymbol{\Theta}}
\newcommand{\bPhi} {\boldsymbol{\Phi}}
\newcommand{\bPsi} {\boldsymbol{\Psi}}
\newcommand{\bRho} {\boldsymbol{\Rho}}
\newcommand{\btheta} {\boldsymbol{\theta}}
\newcommand{\bxi} {\boldsymbol{\xi}}
\newcommand{\bpsi} {\boldsymbol{\psi}}
\newcommand{\bmu} {\boldsymbol{\mu}}
\newcommand{\bzeta} {\boldsymbol{\zeta}}
\newcommand{\bGamma} {\boldsymbol{\Gamma}}
\newcommand{\bLambda} {\boldsymbol{\Lambda}}
\newcommand{\bC}{{\mathbf C}}
\newcommand{\bD}{{\mathbf D}}
\newcommand{\bzero}{{\mathbf 0}}
\newcommand{\bnu}{\boldsymbol{\nu}}
\newcommand{\diff}{\nabla}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  Other mathematical symbols                     %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bbox}{\hfill $\Box$}
\newcommand{\inte}{\int_{-\infty}^{+\infty}}
\newcommand{\rr}{\hbox{$\hskip .1em R\hskip -1.0em\relax I\hskip 0.50em$}}
\newcommand{\sI}{{\cal I}}
\newcommand{\scon}{\stackrel{a.s.}{\longrightarrow}}
\newcommand{\pcon}{\stackrel{P}{\longrightarrow}}
\newcommand{\wcon}{\stackrel{D}{\longrightarrow}}
\newcommand{\asim}{\stackrel{a}{\sim}}
\newcommand{\vs}{\quad \longleftrightarrow \quad }
% \newcommand{\qed}{\hfill $\Box$ \vspace{1mm}}
% \newcommand{\qed}{\hfill $\blacksquare$ \vspace{3mm}}
\newcommand{\calI}{{\mathcal I}}
\newcommand{\calD}{{\mathcal D}}
\newcommand{\calJ}{{\mathcal J}}
\newcommand{\calL}{{\mathcal L}}
\newcommand{\calX}{{\mathcal X}}
\newcommand{\calY}{{\mathcal Y}}
\newcommand{\calZ}{{\mathcal Z}}
\newcommand{\calR}{{\mathcal R}}
\newcommand{\calU}{{\mathcal U}}
\newcommand{\calV}{{\mathcal V}}
\newcommand{\calW}{{\mathcal W}}
\newcommand{\calF}{{\mathcal F}}
\newcommand{\calH}{{\mathcal H}}
\newcommand{\calM}{{\mathcal M}}
\newcommand{\calN}{{\mathcal N}}
\newcommand{\calA}{{\mathcal A}}
\newcommand{\calS}{{\mathcal S}}
\newcommand{\calT}{{\mathcal T}}
\newcommand{\calB}{{\mathcal B}}
\newcommand{\calE}{{\mathcal E}}
\newcommand{\calC}{{\mathcal C}}
\newcommand{\tqn}{\tilde{Q}_T}
\newcommand{\hbeta}{\hat{\beta}}
\newcommand{\RR}{\EuScript R}
\newcommand{\RO}{\EuScript O}
% \newcommand{\SS}{\EuScript S}
\newcommand{\K}{\EuScript K}
\newcommand{\euS}{\EuScript S}
\newcommand{\Z}{\EuScript Z}
\newcommand{\C}{\EuScript C}
\newcommand{\M}{\EuScript M}
\newcommand{\norm}[1]{\| #1 \|}
\def\6bullets{\bullet\bullet\bullet\bullet\bullet\bullet}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Euler math fonds: normal and bold under package euscript
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\eulA}{\EuScript A}
\newcommand{\eulB}{\EuScript B}
\newcommand{\eulC}{\EuScript C}
\newcommand{\eulD}{\EuScript D}
\newcommand{\eulE}{\EuScript E}
\newcommand{\eulF}{\EuScript F}
\newcommand{\eulG}{\EuScript G}
\newcommand{\eulH}{\EuScript H}
\newcommand{\eulI}{\EuScript I}
\newcommand{\eulJ}{\EuScript J}
\newcommand{\eulK}{\EuScript K}
\newcommand{\eulL}{\EuScript L}
\newcommand{\eulM}{\EuScript M}
\newcommand{\eulN}{\EuScript N}
\newcommand{\eulO}{\EuScript O}
\newcommand{\eulP}{\EuScript P}
\newcommand{\eulQ}{\EuScript Q}
\newcommand{\eulR}{\EuScript R}
\newcommand{\eulS}{\EuScript S}
\newcommand{\eulT}{\EuScript T}
\newcommand{\eulU}{\EuScript U}
\newcommand{\eulV}{\EuScript V}
\newcommand{\eulW}{\EuScript W}
\newcommand{\eulX}{\EuScript X}
\newcommand{\eulY}{\EuScript Y}
\newcommand{\eulZ}{\EuScript Z}

\DeclareMathAlphabet\EuScriptBF{U}{eus}{b}{n}
\newcommand{\eulbA}{\EuScriptBF A}
\newcommand{\eulbB}{\EuScriptBF B}
\newcommand{\eulbC}{\EuScriptBF C}
\newcommand{\eulbD}{\EuScriptBF D}
\newcommand{\eulbE}{\EuScriptBF E}
\newcommand{\eulbF}{\EuScriptBF F}
\newcommand{\eulbG}{\EuScriptBF G}
\newcommand{\eulbH}{\EuScriptBF H}
\newcommand{\eulbI}{\EuScriptBF I}
\newcommand{\eulbJ}{\EuScriptBF J}
\newcommand{\eulbK}{\EuScriptBF K}
\newcommand{\eulbL}{\EuScriptBF L}
\newcommand{\eulbM}{\EuScriptBF M}
\newcommand{\eulbN}{\EuScriptBF N}
\newcommand{\eulbO}{\EuScriptBF O}
\newcommand{\eulbP}{\EuScriptBF P}
\newcommand{\eulbQ}{\EuScriptBF Q}
\newcommand{\eulbR}{\EuScriptBF R}
\newcommand{\eulbS}{\EuScriptBF S}
\newcommand{\eulbT}{\EuScriptBF T}
\newcommand{\eulbU}{\EuScriptBF U}
\newcommand{\eulbV}{\EuScriptBF V}
\newcommand{\eulbW}{\EuScriptBF W}
\newcommand{\eulbX}{\EuScriptBF X}
\newcommand{\eulbY}{\EuScriptBF Y}
\newcommand{\eulbZ}{\EuScriptBF Z}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  Math script fonts under package mathrsfs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mathA}{\mathscr A}
\newcommand{\mathB}{\mathscr B}
\newcommand{\mathC}{\mathscr C}
\newcommand{\mathD}{\mathscr D}
\newcommand{\mathE}{\mathscr E}
\newcommand{\mathF}{\mathscr F}
\newcommand{\mathG}{\mathscr G}
\newcommand{\mathH}{\mathscr H}
\newcommand{\mathI}{\mathscr I}
\newcommand{\mathJ}{\mathscr J}
\newcommand{\mathK}{\mathscr K}
\newcommand{\mathL}{\mathscr L}
\newcommand{\mathM}{\mathscr M}
\newcommand{\mathN}{\mathscr N}
\newcommand{\mathO}{\mathscr O}
\newcommand{\mathP}{\mathscr P}
\newcommand{\mathQ}{\mathscr Q}
\newcommand{\mathR}{\mathscr I}
\newcommand{\mathS}{\mathscr S}
\newcommand{\mathT}{\mathscr T}
\newcommand{\mathU}{\mathscr U}
\newcommand{\mathV}{\mathscr V}
\newcommand{\mathW}{\mathscr W}
\newcommand{\mathX}{\mathscr X}
\newcommand{\mathY}{\mathscr Y}
\newcommand{\mathZ}{\mathscr Z}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  Some useful journal names
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\CSDA{{\sl Computational Statistics and Data Analysis}}
\def\JRSSB{{\sl Journal of the Royal Statistical Society}, {\bf B}}
\def\JCGS{{\sl Journal of Computational and Graphical Statistics}}
\def\JBES{{\sl Journal of Business \& Economic Statistics}}
\def\RES{{\sl The Review of Economics and Statistics}}
\def\JRSSA{{\sl Journal of the Royal Statistical Society}, {\bf A}}
\def\JRSSC{{\sl Journal of the Royal Statistical Society}, {\bf C}}
\def\BKA{{\sl Biometrika}}
\def\JASA{{\sl Journal of the American Statistical Association}}
\def\JMLR{{\sl Journal of Machine Learning Research}}
\def\BCS{{\sl Biometrics}}
\def\SS{{\sl Statistica Sinica}}
\def\JAP{{\sl Journal of Applied Probability}}
\def\AAP{{\sl Advances in Applied Probability}}
\def\AS{{\sl The Annals of Statistics}}
\def\JMA{{\sl Journal of multivariate analysis}}
\def\AP{{\sl The Annals of Probability}}
\def\AoAP{{\sl The Annals of Applied Probability}}
\def\AoAS{{\sl The Annals of Applied Statistics}}
\def\SPA{{\sl Stochastic Processes and Their Applications}}
\def\TPA{{\sl Theory of Probability and its Applications}}
\def\JSPI{{\sl Journal of Statistical Planning and Inference}}
\def\JNS{{\sl Journal of Nonparametric Statistics}}
\def\JCGS{{\sl Journal of Computational and Graphical Statistics}}
\def\ET{{\sl Econometric Theory}}
\def\JOE{{\sl Journal of Econometrics}}
\def\JTSA{{\sl Journal of Time Series Analysis}}
\def\SJS{{\sl Scandinavian Journal of Statistics}}
\def\ISR{{\sl International Statistical Review}}
\def\ANZJS{{\sl Australian \& New Zealand Journal of Statistics}}
\def\JE{{\sl Journal of Econometrics}}
\def\SPL{{\sl Statistics and Probability Letters}}
\def\ZW{{\sl Zeitschrift f{\" u}r Wahrscheinlichkeitstheorie und verwandte Gebiete}}
\def\AMS{{\sl The Annals of Mathematical Statistics}}

